Body Schema Acquisition through Active Learning

We present an active learning algorithm for the problem of body schema learning, i.e. estimating a kinematic model of a serial robot. The learning process is done online using Recursive Least Squares (RLS) estimation, which outperforms gradient methods usually applied in the literature. In addiction, the method provides the required information to apply an active learning algorithm to find the optimal set of robot configurations and observations to improve the learning process. By selecting the most informative observations, the proposed method minimizes the required amount of data. We have developed an efficient version of the active learning algorithm to select the points in real-time. The algorithms have been tested and compared using both simulated environments and a real humanoid robot.

==> cost.tex <==

\section{Online POMDP formulation}
\label{sec:activelearning}
	
From the previous Section, we know how to improve th estimation of the parameters with new data. Now we want to choose a sequence of actions that improves this estimation as fast as possible. In this Bayesian experimental design problem, we want to select a set of inputs, or observations, that optimize some utility function $U(\widehat{\x})$, representing an improvement in the estimation quality.

This optimal set of positions $\thetav$ is called a control policy $\pi$. This policy is thus found by minimizing an utility function, that in our case is represented by a quadratic loss function \cite{Chaloner:1995}:
%
\begin{equation}
C_{AMSE}^{\pi}=\ex_{p(\x,\y_{1:\T}|\mbs{\pi})}
\left[(\widehat{\x}_\T-\x)^T (\widehat{\x}_\T-\x) \right]
\end{equation}
%
where $\widehat{\x}_t=\ex_{p(\x|\y_{1:t},\mbs{\pi})}[\x]$. The expectation
is with respect to $p(\x,\y_{1:\T}|\mbs{\pi}) \propto p(\x_0)\prod_{t=1}^{\T}
p(\y_t|\x)$, $\pi(\thetav)$ denotes the policy parameterized by the
configuration way-points $\thetav_i \in \mathbb{R}^{n_\theta}$, $\x_t\in
\mathbb{R}^{n_x}$ is the parameters of the robot (link translation and
rotations) at time $t$, $\y_{1:\T}=\{\y_1,\y_2, \ldots, \y_\T\} \in
\mathbb{R}^{n_y \T}$ is the history of observations for $\T$ steps and
$\widehat{\x}_t$ is the posterior estimate of the state at time $t$. Note that
the true parameters $\x$ and observations are unknown in advance and so one has
to marginalize over them. 

To solve this problem we have to compute the posterior of the parameters and,
since the models are not linear-Gaussian and the cost depends on the belief,
the cost function is not quadratic. Therefore, one cannot use standard
linear-quadratic-Gaussian (LQG) controllers to solve our problem, see
\cite{Bertsekas:1995}. Also, since the action and parameter spaces are
large-dimensional and continuous, one cannot use methods based on discretization
of the problem \cite{Smallwood:1973}.

The algorithm proceeds as follows (see \cite{MartinezCantin07RSS} for details).
First we initial the parameters in a given hypercube, when a new observation
comes we use Eq. \ref{eq:updatep} to update the estimation. When we want to
decide what point to explore next (the policy) we have to perform several steps.
The initial policy is set either randomly \footnote{In practice, we use latin
hypercube sampling, which provides optimal sampling of the
parameter space with uninformative prior.} or using prior knowledge. This policy is simulated using the current distribution of the parameters to yield the ***cost****, we repeat this process several times. With this data we perform an initial estimation of the function $C_{AMSE}^{\pi}$. As this may result in a computational expensive process, we use active learning to generate new policy points to improve the estimation of that function. When a desired accuracy is reached (or the a given time slot), we search for the minimum of that function that gives the policy that best improves the parameters. 

Note that we are applying active learning at two levels. One to select policies that best improve the parameters. To do this we need to estimate a value function and an active method is done to improve the accuracy of this function.


%Having restricted the problem to one of finding the best estimate of the robot
%parameters $\x$, we have to find the optimal set of positions $\thetav$ defined
%by a control policy $\pi$. In orden to find the optimal policy, a quadratic loss
%function \cite{Chaloner:1995} is the natural approach:
%\begin{equation}
%C_{AMSE}^{\pi}=\ex_{p(\x,\y_{1:\T}|\mbs{\pi})}
%\left[(\widehat{\x}_\T-\x)^T (\widehat{\x}_\T-\x) \right]
%\end{equation}
%where $\widehat{\x}_t=\ex_{p(\x|\y_{1:t},\mbs{\pi})}[\x]$. The expectation
%is with respect to $p(\x,\y_{1:\T}|\mbs{\pi}) \propto p(\x_0)\prod_{t=1}^{\T}
%p(\y_t|\x)$, $\pi(\thetav)$ denotes the policy parameterized by the
%configuration way-points $\thetav_i \in \mathbb{R}^{n_\theta}$, $\x_t\in
%\mathbb{R}^{n_x}$ is the parameters of the robot (link translation and
%rotations) at time $t$, $\y_{1:\T}=\{\y_1,\y_2, \ldots, \y_\T\} \in
%\mathbb{R}^{n_y \T}$ is the history of observations for $\T$ steps and
%$\widehat{\x}_t$ is the posterior estimate of the state at time $t$. Note that
%the true parameters $\x$ and observations are unknown in advance and so one has
%to marginalize over them. 
%
%This approach is highly related to the Bayesian experimental design problem.
%The design, or action, consist in selecting a set of inputs, or observations,
%that optimize some utility function $U(\widehat{\x})$, which at the same time,
%is related to the belief function $U(p(\x|\y_{1:t},\mbs{\pi}),\widehat{\x})$.
%It is also related to the belief MDP formulation of POMDPs
%\cite{astroem-markov}, where the reward is defined in terms of the belief.
%However, in our case, the instant reward cannot be integrated from the
%belief.Thus, the cost function hides an enormous degree of complexity. It is a
%function of an \emph{intractable distribution} $p(\x|\y_{1:\T},\mbs{\pi})$
%(also known as the belief). The computation of this belief is explained in
%section \ref{sec:kalman}. 
%
%The general Bayesian network for body schema learning can be seen in figure
%\ref{fig-fullbn}. The main difficulty of the inference problem is due to
%the nonlinearities of the model, which also means that the posterior
%distribution cannot be accurately approximate by a Gaussian.
%
%\begin{figure}
% \centering
% \includegraphics[width=5cm]{figures/fullbayesnet}
% \caption{Bayesian network of SLAM process. Circles represents continuous
%variables and squares are discrete variables. Shaded circles represents observed
%variables. The robot state is represented as $\x$, the observations $\y$, the
%actions $\uv$, the data associations labels $\mathbf{n}$, the map features
%$\thetav$ and the non-stationary policy $\pi$}
% \label{fig-fullbn}
%\end{figure}
%
%
%\subsection{Direct policy search}
%
%Since the models are not linear-Gaussian and the cost depends on the belief, the
%cost function is not quadratic. Therefore, one cannot use standard
%linear-quadratic-Gaussian (LQG) controllers to solve our problem, see
%\cite{Bertsekas:1995}. Moreover, since the action and parameter spaces are
%large-dimensional and continuous, one cannot discretize the problem and use
%closed-loop control as suggested in \cite{Tremois:1999}. That is, the
%discretized partially observed Markov decision process is too large for
%stochastic dynamic programming as suggested in \cite{Smallwood:1973}.
%
%It is important to remark that the cost function depends on the belief
%distribution, therefore, it does not admit close form recursion, and it
%cannot be evaluated instantly for any state and/or action. As a result, we adopt
%the ``episodic'' direct policy search method by \cite{Williams:1992,Ng:2000},
%where the cost is simulated for a given policy and it is compared in terms of
%policies, reseting the state after each policy evaluation.
%
%Due to the enormous complexity of the belief space, defining a policy for
%every belief state is intractable. To aleviate this issue, one can consider
%that the policy is nonstationary, i.e., it depends on the observation gathered
%up to the current decision. Thus, our policy learning method is intended to work
%online, providing a good policy in a small temporal horizon and recomputing the
%policy when new observations are available \cite{Ross08jair}.
%
%In particular, the initial policy is set either randomly\footnote{In practice,
%we use latin hypercube sampling, which provides optimal sampling of the
%parameter space with uninformative prior.} or using prior knowledge. Given this
%policy, we conduct simulations to estimate the cost functions. Then, we update
%the policy parameters and iterate with the goal of minimizing the cost function.
%The pseudocode for this controller is shown in figure~\ref{fig:approach}.
%
%To visualize the complexity of the optimizing the cost function, every episode,
%that is, every policy evaluation, involves computing the posterior distribution
%of the robot parameters}. Then, the belief is reseted and a new policy is
%evaluated. The main advantage and limitation of standard policy search
%algorithms is rooted on its property that observations of one episode do not
%affect the reward of other episodes. This simplicity also implies that a value
%function cannot be learnt. Then, wasting the information gathered in previous
%episodes. Our active policy learning method overcome this limitation by fitting
%a model directly on the policy parameters space to reduce the number of policy
%evaluations.
%
%
%%%% TFS pseudo code ---------------------------------------------------------
%\begin{figure}
%\begin{center}
%\par \hspace{-.5mm} \framebox[0.98\linewidth][l]{
%\begin{minipage}[l]{0.93\linewidth}\vspace{2mm}
% {\footnotesize
%
\begin{figure}
\begin{center}
\par \hspace{-.5mm} \framebox[0.98\linewidth][l]{
\begin{minipage}[l]{0.93\linewidth}\vspace{2mm}
 {\footnotesize

\begin{enumerate}
\item Choose an initial policy $\pi_0$.
\item For $j=1:MaxNumberOfPolicySearchIterations$
\item Simulate the robot trajectory to the configuration determined by the
policy $\pi_j$.
\item Generate observations based on the current estimate and the
observation model $\y_t^{(i)}\sim p(\y_t|,\x_{t}^{(i)})$.
\item Compute the posterior distribution $p(\x_t|\y_{1:t}^{(i)})$ using the
algorithm in section \ref{sec:kalman}.
\item Evaluate the approximate cost function of equation~(\eqref{eqn:amsecost})
using the simulated trajectory.
\item Use the active learning algorithm described in section~\ref{sec:apl}, to
generate the new policy $\pi_{j+1}$. The choice of the new policy is governed by
our desire to exploit and our need to explore the space of policies (navigation
paths). In particular, we give preference to policies for which we expect the
cost to be minimized and to policies where we have high uncertainty about what
the cost might be.
\end{enumerate}

 \vspace{2mm} \small}
\end{minipage}}
\end{center}
\caption{The active policy learning algorithm for body schema learning. It is
implicit in the pseudo-code that we use common random numbers so as to reduce
variance.}
\label{fig:approach}
\end{figure}%%%%%%%%%%%%%% ---------------------------------------------------------


==> optimization.tex <==
\section{Global Optimization for Action Selection}

Having restricted the problem of selecting the most informative action to one of finding the global minimum of a cost function, we can use many of the existing techniques for efficient global optimization. There is always a trade-off between exploration and exploitation. Global optimization methods require dense sampling of the whole space in order to guarantee global convergence. This may result in poor perfomance of local refinement. In order to maximize the performance, we can identify the subsequent properties of our cost function:
\begin{itemize}
 \item Since all the functions involved are continous, except for the field of view and motor boundaries, the cost function is continous or, at least, locally continuous.
 \item In the same line of though, we can assume that the cost function is smooth, at least, in the neighbourhood to the global minimum.
 \item Evaluate the cost function is expensive. Therefore, the number of iterations and function evaluations should remain low.
 \item It is non-trivial to obtain the gradient of the cost function.
\end{itemize}

This setup is perfect for Lipschitzian or Bayesian optimization.

\subsection{Lipschitzian optimization}

Lipschitzian optimization is a simple but powerfull method for global optimization that relies on a deterministic search of in a multidimensional hypercube. Any Lipschitizian algorithm assumes that the cost function satisfies
\begin{equation}
 |f(\x) - f(\x')| \leqslant K|\x-\x'| \; \;\;\; \forall \x, \x' \in S
\end{equation}
for a positive constant $K$ and any closed set $S$. This assumption can be trivially obtained from our previous assumptions and can be used to set a lower bound on the function for any closed set. The lower bound is used to divide the set in smaller sets and refine the search recursively. The algorithm presented in \cite{Jones:1993} (called DIRECT) uses hypercubes as the closed sets, and the center point of the set is used for evaluation. The advantage of using the central point is twofold: (i) it requires only one point despite the number of dimension, contrary to the $2^n$ points required to evaluated the endpoints, (ii) it allows to compare the lower bound of two subsets for any Lipschitz constant $K$, therefore, it can be unknown in advance.

Once we have the bound, we can identify pontentially optimal subsets, that is, the hyperrectangles $j \in [1 \cdots m]$ that satisfy
\begin{align}
 \exists \tilde{K} > 0 \mid f(c_j) - \tilde{K}d_j &\leqslant f(c_i) - \tilde{K}d_i  \; \;\;\; \forall i= 1 \cdots m \\
f(c_j) - \tilde{K}d_j &\leqslant f_{min} - \epsilon |f_{min}|
\end{align}
where $c_i$ is the central point of hyperrectangle $i$ and $f_{min}$ is the minimum value found so far. The first condition selects all potentially optimal points for any positive $\tilde{K}$ by just selecting the piecewise linear function that conects the points with minimum $f(c)$ for any $d_j$. Figure 5 and 6 of \cite{Jones:1993} provides a simple intuition of this method. The second condition guarantees that any iteration, there is a non-trivial improvement in order to guarantee global convergency and to avoid being stuck in flat local minima. In our robotics setup, this condition is specially critical, since small improvements in the cost functions are pointless in terms of learning, while global exploration is fundamental to find good policies.

One of the main issues of active learning in robotics, is that data selection has to be computed in a reasonable time. That is, the overall cost cannot exceed the cost of processing large datasets at random or even worse, the time to sweep the whole space with the robot. Thus, we require to set a budget for the optimization process. Under that circumstances, it seems more suitable to use the extension of the DIRECT algorithm, called DIRECT-l \cite{Gablonksy:2001} which reduces the computational cost of every sweep over the function by clustering the rectangles.

\subsection{Bayesian optimization}

Since our cost function is based on the lookahead simulation and computation of the posterior distribution of a high dimensional set of parameters, the evaluation of every point is a time consuming process. Furthermore, as said in the previous section, there is a computation budget. Therefore, we need to reduce the number of function evaluations during optimization.

An efficient method for global optimization of expensive functions is Bayesian optimization. Based on the work of Kushner \cite{Kushner:1964} and Mockus et al. \cite{Mockus78}, it computes a posterior distribution over all possible cost functions given all the evaluations so far. Then, it selects the next point based on a statistical measure of improving the search. It also 
